Weakly-Supervised Audio-Visual Segmentation

Audio-visual segmentation is a challenging task that aims to predict pixel-level masks for sound sources in a video. Previous work applied a comprehensive manually designed architecture with countless pixel-wise accurate masks as supervision. However, these pixel-level masks are expensive and not available in all cases. In this work, we aim to simplify the supervision as the instance-level annotation, i.e., weakly-supervised audio-visual segmentation. We present a novel Weakly-Supervised Audio-Visual Segmentation framework, namely WS-AVS, that can learn multi-scale audio-visual alignment with multi-scale multiple-instance contrastive learning for audio-visual segmentation. Extensive experiments on AVSBench demonstrate the effectiveness of our WS-AVS in the weakly-supervised audio-visual segmentation of single-source and multi-source scenarios.

==> SECTIONS/10_Introduction/title_image.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\textwidth]{figs/title_image.pdf}
\caption{Comparison of audio-visual segmentation~\cite{zhou2022avs}, and the proposed weakly-supervised audio-visual segmentation.
}
\label{fig: title_img}
\end{figure}
